Relaxed Attention: A Simple Method to Boost Performance of End-to-End Automatic Speech Recognition

Recently, attention-based encoder-decoder (AED) models have shown high performance for end-to-end automatic speech recognition (ASR) across several tasks. Addressing overconfidence in such models, in this paper we introduce the concept of relaxed attention, which is a simple gradual injection of a uniform distribution to the encoder-decoder attention weights during training that is easily implemented with two lines of code. We investigate the effect of relaxed attention across different AED model architectures and two prominent ASR tasks, Wall Street Journal (WSJ) and Librispeech. We found that transformers trained with relaxed attention outperform the standard baseline models consistently during decoding with external language models. On WSJ, we set a new benchmark for transformer-based end-to-end speech recognition with a word error rate of 3.65%, outperforming state of the art (4.20%) by 13.1% relative, while introducing only a single hyperparameter.

==> macros/fewmathmacros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematical macros, only a few of them
%
% Tim Fingscheidt IfN / TU Braunschweig, 2021-03-02
%

\newcommand{\ACC}{\mathrm{ACC}}         % Accuracy
\newcommand{\FP}{\mathrm{FP}}           % # of false positives
\newcommand{\FN}{\mathrm{FN}}           % # of false negatives
\newcommand{\TP}{\mathrm{TP}}           % # of true positives
\newcommand{\TN}{\mathrm{TN}}           % # of true negatives
\newcommand{\FPR}{\mathrm{FPR}}         % False positive rate
\newcommand{\FAR}{\mathrm{FAR}}         % False acceptance rate = FPR
\newcommand{\FNR}{\mathrm{FNR}}         % False negative rate
\newcommand{\FRR}{\mathrm{FRR}}         % False rejection rate = FNR
\newcommand{\TPR}{\mathrm{TPR}}         % True positive rate = hit rate = recall
\newcommand{\TNR}{\mathrm{TNR}}         % True negative rate
\newcommand{\EER}{\mathrm{EER}}         % Equal Error Rate
\newcommand{\ER}{\mathrm{ER}}           % Error Rate
\newcommand{\PRECISION}{\mathrm{Precision}} % Precision
\newcommand{\RECALL}{\mathrm{Recall}}       % Recall = TPR
\newcommand{\FMEASURE}{\mathrm{F1}}         % F1 score, F-measure
\newcommand{\mIoU}{\mathrm{mIoU}}           % # Mean intersection over Union
\newcommand{\SSIM}{\mathrm{SSIM}}           % # Structural similarity
\newcommand{\MSSSIM}{\mathrm{MS\!\!\--\!\!SSIM}} % # Multi-scale structural similarity
\newcommand{\MSE}{\mathrm{MSE}}             % Mean Square Error
\newcommand{\SNRSEG}{\mathrm{SNR}_{\mathrm{seg}}}
\newcommand{\SNR}{\mathrm{SNR}}
\newcommand{\PSNR}{\mathrm{PSNR}}
\newcommand{\FR}{\mathrm{FR}}				% Fooling rate

\newcommand{\VEC}[1]{\mathbf{#1}}          % Vector
\newcommand{\VECG}[1]{\boldsymbol{#1}}     % Vector with Greek letter
\newcommand{\MAT}[1]{\mathbf{#1}}          % Matrix
\newcommand{\MATG}[1]{\boldsymbol{#1}}     % Matrix with Greek letter

% Number sets: ------------------------------------------------
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\G}{\mathbb{G}}

% Transposed "T": ------------------------------------------------------
\newcommand{\T}[0]{\mathsf{T}}

% Transformations: -------------------------------------------------------
\newcommand{\invfourier}[0]{\bullet \hspace{-1.7mm} - \hspace{-1.7mm} \circ}
\newcommand{\fourier}[0]{\circ \hspace{-1.7mm} - \hspace{-1.7mm} \bullet}
\newcommand{\DFT}[1]{{\mathrm DFT}\{#1\}}
\newcommand{\DCT}[1]{{\mathrm DCT}\{#1\}}


\newcommand{\PROBD}[1][]{{\mathrm p_{#1}}} % p( ), Probability Density Function
\newcommand{\PROB}[0]{{\mathrm P}}         % P( ), Probability
\newcommand{\EXPVAL}{\mathbb{E}}           % NEW: Expectation value


